Optimizing Two-Truck Platooning with Deadlines

We study a transportation problem where two heavy-duty trucks travel across the national highway from separate origins to destinations, subject to individual deadline constraints. Our objective is to minimize their total fuel consumption by jointly optimizing path planning, speed planning, and platooning configuration. Such a two-truck platooning problem is pervasive in practice yet challenging to solve due to hard deadline constraints and enormous platooning configurations to consider. We first leverage a unique problem structure to significantly simplify platooning optimization and present a novel formulation. We prove that the two-truck platooning problem is weakly NP-hard and admits a Fully Polynomial Time Approximation Scheme (FPTAS). The FPTAS can achieve a fuel consumption within a ratio of $(1+\epsilon)$ to the optimal (for any $\epsilon>0$) with a time complexity polynomial in the size of the transportation network and $1/\epsilon$. These results are in sharp contrast to the general multi-truck platooning problem, which is known to be APX-hard and repels any FPTAS. As the FPTAS still incurs excessive running time for large-scale cases, we design an efficient dual-subgradient algorithm for solving large-/national- scale instances. It is an iterative algorithm that always converges. We prove that each iteration only incurs polynomial-time complexity, albeit it requires solving an integer linear programming problem optimally. We characterize a condition under which the algorithm generates an optimal solution and derive a posterior performance bound when the condition is not met. Extensive simulations based on real-world traces show that our joint solution of path planning, speed planning, and platooning saves up to $24\%$ fuel as compared to baseline alternatives.

==> tex/highlights.tex <==
\begin{highlights}

% \item We show that the two-truck platooning problem of minimizing fuel consumption subject to individual deadline constraints, considering path planning, speed planning, and platooning configuration.

\item We show that the two-truck platooning problem is NP-hard, but only in the weak sense. 

% This contrasts with the general multi-truck platooning problem, which is at least NP-hard in the strong sense. 


% \item A new formulation is proposed for the two-truck platooning problem. We show that the problem is fundamentally NP-hard.

% small scale 
% \item We develop an effective fully polynomial-time approximation algorithm for solving small-/medium- scale instances. 

% but admits an approximation algorithm with an approximation ratio of (1+$\epsilon$) for any $\epsilon>0$ and a polynomial-time complexity.

% \item We develop an efficient dual-subgradient algorithm for solving large-/national- scale two-truck platooning instances.

\item We develop efficient algorithms for the two-truck platooning problem with performance guarantees. 

\item Simulations based on real-world traces show that our solutions save up to $24\%$ more fuel than baselines adapted from state-of-the-art schemes.

% \item We study the two-truck platooning problem of minimizing fuel consumption subject to individual deadline constraints, taking into account path planning, speed planning, and platooning configuration.

% % small scale 
% \item We exploit a problem structure to present a new formulation for the problem. We show that the problem is fundamentally NP-hard.

% \item We propose a fully polynomial-time approximation algorithm for small-scale cases.
% % but admits an approximation algorithm with an approximation ratio of (1+$\epsilon$) for any $\epsilon>0$ and a polynomial-time complexity.

% \item We design an efficient dual-subgradient algorithm for solving large-/national- scale instances of two-truck platooning.

% \item Extensive simulations based on real-world traces show that our solution saves up to $24\%$ fuel compared to baselines adapted from state-of-the-art schemes.
\end{highlights}
